A Technique Based on Trade-off Maps to Visualise and Analyse Relationships Between Objectives in Optimisation Problems

Understanding the relationships between objectives in a multiobjective optimisation problem is important for developing tailored and efficient solving techniques. In particular, when tackling combinatorial optimisation problems with many objectives, that arise in real-world logistic scenarios, better support for the decision maker can be achieved through better understanding of the often complex fitness landscape. This paper makes a contribution in this direction by presenting a technique that allows a visualisation and analysis of the local and global relationships between objectives in optimisation problems with many objectives. The proposed technique uses four steps: First, the global pairwise relationships are analysed using the Kendall correlation method; then, the ranges of the values found on the given Pareto front are estimated and assessed; next, these ranges are used to plot a map using Gray code, similar to Karnaugh maps, that has the ability to highlight the trade-offs between multiple objectives; and finally, local relationships are identified using scatter plots. Experiments are presented for three combinatorial optimisation problems: multiobjective multidimensional knapsack problem, multiobjective nurse scheduling problem, and multiobjective vehicle routing problem with time windows . Results show that the proposed technique helps in the gaining of insights into the problem difficulty arising from the relationships between objectives.

==> figures/step1.tex <==
\begin{table}[h]
\centering
\begin{subtable}[b]{0.40\textwidth}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrr}
\multicolumn{1}{c}{Set A} & \multicolumn{1}{c}{A1} & \multicolumn{1}{c}{A2} & \multicolumn{1}{c}{A3} & \multicolumn{1}{c}{A4} & \multicolumn{1}{c}{A5} & \multicolumn{1}{c}{Mean} \\ \hline \hline
$Z_1$-$Z_2$               & -0.15                  & -0.33                  & -0.21                  & -0.39                  & -0.49                  & {\color[HTML]{986536} \textbf{-0.314}}                   \\
$Z_1$-$Z_3$               & -0.02                  & 0.09                   & -0.43                  & -0.34                  & 0.11                   & {\color[HTML]{986536} \textbf{-0.118}}                   \\
$Z_1$-$Z_4$               & -0.21                  & 0.09                   & -0.18                  & 0.20                   & 0.07                   & {\color[HTML]{986536} \textbf{-0.006}}                   \\
$Z_2$-$Z_3$               & -0.30                  & -0.37                  & 0.17                   & 0.01                   & -0.42                  & {\color[HTML]{986536} \textbf{-0.182}}                   \\
$Z_2$-$Z_4$               & 0.06                   & -0.22                  & -0.17                  & -0.41                  & -0.09                  & {\color[HTML]{986536} \textbf{-0.166}}                   \\
$Z_3$-$Z_4$               & -0.25                  & -0.20                  & -0.22                  & -0.26                  & 0.19                   & {\color[HTML]{986536} \textbf{-0.148}}                   \\ \hline \\
\end{tabular}
}
\label{s1A}
\end{subtable}
\begin{subtable}[b]{0.40\textwidth}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrr}
\multicolumn{1}{c}{Set C} & \multicolumn{1}{c}{C1} & \multicolumn{1}{c}{C2} & \multicolumn{1}{c}{C3} & \multicolumn{1}{c}{C4} & \multicolumn{1}{c}{C5} & \multicolumn{1}{c}{Mean} \\ \hline \hline
$Z_1$-$Z_2$ & -0.96	& -0.97	& -0.98	& -0.98	& -0.98 & {\color[HTML]{9A0000} \textbf{-0.974}}\\ 
$Z_1$-$Z_3$ &  0.93	&  0.95	&  0.95	&  0.96	&  0.96 &  {\color[HTML]{036400} \textbf{0.950}}\\ 
$Z_1$-$Z_4$ & -0.93	& -0.92	& -0.92	& -0.97	& -0.95 & {\color[HTML]{9A0000} \textbf{-0.938}}\\ 
$Z_2$-$Z_3$ & -0.96	& -0.96	& -0.97	& -0.97	& -0.96 & {\color[HTML]{9A0000} \textbf{-0.964}}\\ 
$Z_2$-$Z_4$ &  0.95	&  0.92	&  0.93	&  0.96	&  0.94 &  {\color[HTML]{036400} \textbf{0.940}}\\ 
$Z_3$-$Z_4$ & -0.98	& -0.94	& -0.95	& -0.97	& -0.97 & {\color[HTML]{9A0000} \textbf{-0.962}}\\ \hline \\
\end{tabular}
}
\label{s1C}
\end{subtable}
\\ \vfill
\begin{subtable}[b]{0.40\textwidth}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrr}
\multicolumn{1}{c}{Set D} & \multicolumn{1}{c}{D1} & \multicolumn{1}{c}{D2} & \multicolumn{1}{c}{D3} & \multicolumn{1}{c}{D4} & \multicolumn{1}{c}{D5} & \multicolumn{1}{c}{Mean} \\ \hline \hline
$Z_1$-$Z_2$& -0.92& -0.92& -0.94& -0.94& -0.94& {\color[HTML]{9A0000} \textbf{-0.932}}\\ 
$Z_1$-$Z_3$&  0.88&  0.84&  0.88&  0.87&  0.87&  {\color[HTML]{036400} \textbf{0.868}}\\ 
$Z_1$-$Z_4$& -0.84& -0.84& -0.87& -0.87& -0.87& {\color[HTML]{9A0000} \textbf{-0.858}}\\ 
$Z_2$-$Z_3$& -0.87&  0.90& -0.91& -0.90& -0.90& {\color[HTML]{9A0000} \textbf{-0.896}}\\ 
$Z_2$-$Z_4$&  0.82&  0.86&  0.87&  0.87&  0.87&  {\color[HTML]{036400} \textbf{0.858}}\\ 
$Z_3$-$Z_4$& -0.92& -0.93& -0.93&  0.92& -0.92& {\color[HTML]{9A0000} \textbf{-0.924}}\\ \hline
\end{tabular}
}
\label{s1D}
\end{subtable}
\\ \bigskip
\begin{subtable}[b]{0.40\textwidth}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrr}
\multicolumn{1}{c}{Set X} & \multicolumn{1}{c}{X1} & \multicolumn{1}{c}{X2} & \multicolumn{1}{c}{X3} & \multicolumn{1}{c}{X4} & \multicolumn{1}{c}{X5} & \multicolumn{1}{c}{Mean} \\ \hline \hline
$Z_1$-$Z_2$ & -0.26 & -0.29 & -0.13 & -0.24 & -0.32 & {\color[HTML]{986536} \textbf{-0.248}} \\ 
$Z_1$-$Z_3$ & -0.13 & -0.24 & -0.27 & -0.25 & -0.27 & {\color[HTML]{986536} \textbf{-0.232}} \\ 
$Z_1$-$Z_4$ & -0.29 & -0.12 & -0.29 & -0.21 & -0.07 & {\color[HTML]{986536} \textbf{-0.196}} \\ 
$Z_2$-$Z_3$ & -0.25 & -0.13 & -0.26 & -0.23 & -0.19 & {\color[HTML]{986536} \textbf{-0.212}} \\ 
$Z_2$-$Z_4$ & -0.13 & -0.28 & -0.22 & -0.11 & -0.27 & {\color[HTML]{986536} \textbf{-0.202}} \\ 
$Z_3$-$Z_4$ & -0.24 & -0.23 & -0.14 & -0.21 & -0.18 & {\color[HTML]{986536} \textbf{-0.200}} \\ \hline
\end{tabular}
}
\label{s1X}
\end{subtable}
\caption{Results for the pairwise relationship analysis  (1.0 is completely harmonious, -1.0 is completely conflicting).}
\label{step1}
\end{table}

==> figures/step2.tex <==
\begin{table}[!ht]
\centering
\begin{subtable}{0.47\linewidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccccccccc}
\multicolumn{2}{l}{Set A}                                               & {A1}     & {A2}     & {A3}     & {A4}     & {A5}     & {} & {Mean}   \\ \hline\hline
\multicolumn{1}{c}{\multirow{3}{*}{{$Z_1$}}} & {Max}   & 105269          & 105591          & 98845           & 109048          & 98562           &           & 103463.0        \\  
\multicolumn{1}{c}{}                                & {Min}   & 81507           & 84910           & 72393           & 82400           & 78259           &           & 79893.8         \\  
\multicolumn{1}{c}{}                                & {Range} & \textbf{\color[HTML]{986536}{22.6\%}} & \textbf{\color[HTML]{986536}{19.6\%}} & \textbf{\color[HTML]{986536}{26.8\%}} & \textbf{\color[HTML]{986536}{24.4\%}} & \textbf{\color[HTML]{986536}{20.6\%}} & {} & \textbf{\color[HTML]{986536}{22.8\%}} \\ \hline
\multicolumn{1}{c}{\multirow{3}{*}{{$Z_2$}}} & {Max}   & 105565          & 102067          & 101879          & 107485          & 106290          &           & 104657.2        \\ 
\multicolumn{1}{c}{}                                & {Min}   & 84618           & 78862           & 75194           & 78073           & 82345           &           & 79818.4         \\ 
\multicolumn{1}{c}{}                                & {Range} & \textbf{\color[HTML]{986536}{19.8\%}} & \textbf{\color[HTML]{986536}{22.7\%}} & \textbf{\color[HTML]{986536}{26.2\%}} & \textbf{\color[HTML]{986536}{27.4\%}} & \textbf{\color[HTML]{986536}{22.5\%}} & {} & \textbf{\color[HTML]{986536}{23.7\%}} \\ \hline
\multicolumn{1}{c}{\multirow{3}{*}{{$Z_3$}}} & {Max}   & 100267          & 105755          & 106024          & 110554          & 102331          &           & 104986.2        \\  
\multicolumn{1}{c}{}                                & {Min}   & 76363           & 80682           & 78207           & 82257           & 77085           &           & 78918.8         \\ 
\multicolumn{1}{c}{}                                & {Range} & \textbf{\color[HTML]{986536}{23.8\%}} & \textbf{\color[HTML]{986536}{23.7\%}} & \textbf{\color[HTML]{986536}{26.2\%}} & \textbf{\color[HTML]{986536}{25.6\%}} & \textbf{\color[HTML]{986536}{24.7\%}} & {} & \textbf{\color[HTML]{986536}{24.8\%}} \\ \hline
\multicolumn{1}{c}{\multirow{3}{*}{{$Z_4$}}} & {Max}   & 107607          & 110827          & 105888          & 103686          & 106472          &           & 16895.4         \\  
\multicolumn{1}{c}{}                                & {Min}   & 84932           & 88405           & 75817           & 76770           & 86274           &           & 82439.6         \\ 
\multicolumn{1}{c}{}                                & {Range} & \textbf{\color[HTML]{986536}{21.1\%}} & \textbf{\color[HTML]{986536}{20.2\%}} & \textbf{\color[HTML]{986536}{28.4\%}} & \textbf{\color[HTML]{986536}{26.0\%}} & \textbf{\color[HTML]{986536}{19.0\%}} & {} & \textbf{\color[HTML]{986536}{22.9\%}} \\ \hline
\end{tabular}
}
%\subcaption{Set A}
\label{s2A}
\end{subtable}
%\\ \bigskip
\begin{subtable}{0.43\linewidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccccccccc}
\multicolumn{2}{l}{Set B}                                                & {B1}    & {B2}  & {B3}    & {B4}    & {B5}  & {} & {Mean}  \\ \hline\hline
\multicolumn{1}{c}{\multirow{3}{*}{{$Z_1$}}} & {Max}   & 103713         & n/a          & 104141         & 111900         & n/a          &           & 106584.7       \\ 
\multicolumn{1}{c}{}                                & {Min}   & 102748         & n/a          & 104107         & 111622         & n/a          &           & 106159.0       \\ 
\multicolumn{1}{c}{}                                & {Range} & \textbf{\color[HTML]{9A0000}{0.9\%}} & {n/a} & \textbf{\color[HTML]{9A0000}{0.1\%}} & \textbf{\color[HTML]{9A0000}{0.2\%}} & {n/a} & {} & \textbf{\color[HTML]{9A0000}{0.4\%}} \\ \hline
\multicolumn{1}{c}{\multirow{3}{*}{{$Z_2$}}} & {Max}   & 104952         & n/a          & 107233         & 113620         & n/a          &           & 108601.7       \\ 
\multicolumn{1}{c}{}                                & {Min}   & 104410         & n/a          & 106638         & 113496         & n/a          &           & 108181.3       \\ 
\multicolumn{1}{c}{}                                & {Range} & \textbf{\color[HTML]{9A0000}{0.5\%}} & {n/a} & \textbf{\color[HTML]{9A0000}{0.6\%}} & \textbf{\color[HTML]{9A0000}{0.1\%}} & {n/a} & {} & \textbf{\color[HTML]{9A0000}{0.4\%}} \\ \hline
\multicolumn{1}{c}{\multirow{3}{*}{{$Z_3$}}} & {Max}   & 106633         & n/a          & 109010         & 113821         & n/a          &           & 109821.3       \\ 
\multicolumn{1}{c}{}                                & {Min}   & 106274         & n/a          & 108175         & 113479         & n/a          &           & 109309.3       \\ 
\multicolumn{1}{c}{}                                & {Range} & \textbf{\color[HTML]{9A0000}{0.3\%}} & {n/a} & \textbf{\color[HTML]{9A0000}{0.8\%}} & \textbf{\color[HTML]{9A0000}{0.3\%}} & {n/a} & {} & \textbf{\color[HTML]{9A0000}{0.5\%}} \\ \hline
\multicolumn{1}{c}{\multirow{3}{*}{{$Z_4$}}} & {Max}   & 107347         & n/a          & 108361         & 113926         & n/a          &           & 109878.0       \\ 
\multicolumn{1}{c}{}                                & {Min}   & 107025         & n/a          & 107324         & 113663         & n/a          &           & 109337.3       \\ 
\multicolumn{1}{c}{}                                & {Range} & \textbf{\color[HTML]{9A0000}{0.3\%}} & {n/a} & \textbf{\color[HTML]{9A0000}{1.0\%}} & \textbf{\color[HTML]{9A0000}{0.2\%}} & {n/a} & {} & \textbf{\color[HTML]{9A0000}{0.5\%}} \\ \hline
\end{tabular}
}
%\subcaption{Set B}
\label{s2B}
\end{subtable}
%\\ \bigskip
\begin{subtable}{0.45\linewidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccccccccc}
\multicolumn{2}{l}{Set C}                                                & {C1}     & {C2}     & {C3}     & {C4}     & {C5}     & {} & {Mean}   \\ \hline\hline
\multicolumn{1}{c}{\multirow{3}{*}{{$Z_1$}}} & {Max}   & 109142          & 105928          & 114773          & 115084          & 112290          &           & 111443.4        \\ 
\multicolumn{1}{c}{}                                & {Min}   & 34911           & 33631           & 35449           & 35317           & 33157           &           & 34493.0         \\ 
\multicolumn{1}{c}{}                                & {Range} & \textbf{\color[HTML]{036400}{68.0\%}} & \textbf{\color[HTML]{036400}{68.3\%}} & \textbf{\color[HTML]{036400}{69.1\%}} & \textbf{\color[HTML]{036400}{69.3\%}} & \textbf{\color[HTML]{036400}{70.5\%}} & {} & \textbf{\color[HTML]{036400}{69.0\%}} \\ \hline
\multicolumn{1}{c}{\multirow{3}{*}{{$Z_2$}}} & {Max}   & 111124          & 109863          & 110290          & 114339          & 112559          &           & 111635.0        \\ 
\multicolumn{1}{c}{}                                & {Min}   & 37928           & 36764           & 33189           & 30491           & 32431           &           & 34160.6         \\ 
\multicolumn{1}{c}{}                                & {Range} & \textbf{\color[HTML]{036400}{65.9\%}} & \textbf{\color[HTML]{036400}{66.5\%}} & \textbf{\color[HTML]{036400}{69.9\%}} & \textbf{\color[HTML]{036400}{73.3\%}} & \textbf{\color[HTML]{036400}{71.2\%}} & {} & \textbf{\color[HTML]{036400}{69.4\%}} \\ \hline
\multicolumn{1}{c}{\multirow{3}{*}{{$Z_3$}}} & {Max}   & 109775          & 104817          & 113400          & 115214          & 112467          &           & 111134.6        \\ 
\multicolumn{1}{c}{}                                & {Min}   & 35859           & 33066           & 35326           & 35508           & 33004           &           & 34552.6         \\ 
\multicolumn{1}{c}{}                                & {Range} & \textbf{\color[HTML]{036400}{67.3\%}} & \textbf{\color[HTML]{036400}{68.5\%}} & \textbf{\color[HTML]{036400}{68.8\%}} & \textbf{\color[HTML]{036400}{69.2\%}} & \textbf{\color[HTML]{036400}{70.2\%}} & {} & \textbf{\color[HTML]{036400}{68.9\%}} \\ \hline
\multicolumn{1}{c}{\multirow{3}{*}{{$Z_4$}}} & {Max}   & 109569          & 108055          & 109242          & 113106          & 113391          &           & 110272.6        \\ 
\multicolumn{1}{c}{}                                & {Min}   & 38774           & 37107           & 34277           & 32074           & 34062           &           & 35258.8         \\ 
\multicolumn{1}{c}{}                                & {Range} & \textbf{\color[HTML]{036400}{64.6\%}} & \textbf{\color[HTML]{036400}{65.7\%}} & \textbf{\color[HTML]{036400}{68.6\%}} & \textbf{\color[HTML]{036400}{71.6\%}} & \textbf{\color[HTML]{036400}{69.4\%}} & {} & \textbf{\color[HTML]{036400}{68.0\%}} \\ \hline
\end{tabular}
}
%\subcaption{Set C}
\label{s2C}
\end{subtable}
%\\ \bigskip
\begin{subtable}{0.45\linewidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccccccccc}

\multicolumn{2}{l}{Set D}                                               & {D1}     & {D2}     & {D3}     & {D4}     & {D5}     & {} & {Mean}   \\ \hline\hline
\multicolumn{1}{c}{\multirow{3}{*}{{$Z_1$}}} & {Max}   & 186945          & 190209          & 188157          & 170337          & 179792          &           & 183088.0        \\ 
\multicolumn{1}{c}{}                                & {Min}   & 58152           & 65554           & 69709           & 53810           & 64747           &           & 62394.4         \\ 
\multicolumn{1}{c}{}                                & {Range} & \textbf{\color[HTML]{036400}{68.9\%}} & \textbf{\color[HTML]{036400}{65.5\%}} & \textbf{\color[HTML]{036400}{63.0\%}} & \textbf{\color[HTML]{036400}{68.4\%}} & \textbf{\color[HTML]{036400}{64.0\%}} & {} & \textbf{\color[HTML]{036400}{65.9\%}} \\ \hline
\multicolumn{1}{c}{\multirow{3}{*}{{$Z_2$}}} & {Max}   & 180305          & 188813          & 197847          & 183889          & 191691          &           & 188509.0        \\ 
\multicolumn{1}{c}{}                                & {Min}   & 64198           & 58680           & 68608           & 55859           & 63604           &           & 62189.8         \\ 
\multicolumn{1}{c}{}                                & {Range} & \textbf{\color[HTML]{036400}{64.4\%}} & \textbf{\color[HTML]{036400}{68.9\%}} & \textbf{\color[HTML]{036400}{65.3\%}} & \textbf{\color[HTML]{036400}{69.6\%}} & \textbf{\color[HTML]{036400}{66.8\%}} & {} & \textbf{\color[HTML]{036400}{67.0\%}} \\ \hline
\multicolumn{1}{c}{\multirow{3}{*}{{$Z_3$}}} & {Max}   & 185349          & 189131          & 187175          & 169153          & 180283          &           & 182218.2        \\ 
\multicolumn{1}{c}{}                                & {Min}   & 56697           & 63717           & 68430           & 52449           & 67272           &           & 61713.0         \\ 
\multicolumn{1}{c}{}                                & {Range} & \textbf{\color[HTML]{036400}{69.4\%}} & \textbf{\color[HTML]{036400}{66.3\%}} & \textbf{\color[HTML]{036400}{63.4\%}} & \textbf{\color[HTML]{036400}{69.0\%}} & \textbf{\color[HTML]{036400}{62.7\%}} & {} & \textbf{\color[HTML]{036400}{66.1\%}} \\ \hline
\multicolumn{1}{c}{\multirow{3}{*}{{$Z_4$}}} & {Max}   & 182878          & 188835          & 196048          & 182326          & 190441          &           & 188105.6        \\ 
\multicolumn{1}{c}{}                                & {Min}   & 66673           & 61884           & 70145           & 59158           & 66344           &           & 64840.8         \\ 
\multicolumn{1}{c}{}                                & {Range} & \textbf{\color[HTML]{036400}{63.5\%}} & \textbf{\color[HTML]{036400}{67.2\%}} & \textbf{\color[HTML]{036400}{64.2\%}} & \textbf{\color[HTML]{036400}{67.6\%}} & \textbf{\color[HTML]{036400}{65.2\%}} & {} & \textbf{\color[HTML]{036400}{65.5\%}} \\ \hline
\end{tabular}
}
%\subcaption{Set D}
\label{s2D}
\end{subtable}
\\ \bigskip
\begin{subtable}{\linewidth}
\centering
\resizebox{0.45\linewidth}{!}{%
\begin{tabular}{ccccccccc}

\multicolumn{2}{l}{Set X}                                                & {X1}     & {X2}     & {X3}     & {X4}     & {X5}     & {} & {Mean}   \\ \hline\hline
\multicolumn{1}{c}{\multirow{3}{*}{{$Z_1$}}} & {Max}   & 29105           & 30825           & 29173           & 29906           & 30536           &           & 29909.0         \\ 
\multicolumn{1}{c}{}                                & {Min}   & 4930            & 3703            & 5317            & 4685            & 4429            &           & 4612.8          \\ 
\multicolumn{1}{c}{}                                & {Range} & \textbf{\color[HTML]{036400}{83.1\%}} & \textbf{\color[HTML]{036400}{88.0\%}} & \textbf{\color[HTML]{036400}{81.8\%}} & \textbf{\color[HTML]{036400}{84.3\%}} & \textbf{\color[HTML]{036400}{85.5\%}} & {} & \textbf{\color[HTML]{036400}{84.6\%}} \\ \hline
\multicolumn{1}{c}{\multirow{3}{*}{{$Z_2$}}} & {Max}   & 28885           & 30180           & 29314           & 28990           & 31422           &           & 29758.2         \\ 
\multicolumn{1}{c}{}                                & {Min}   & 4706            & 4506            & 5024            & 4027            & 4190            &           & 4490.6          \\ 
\multicolumn{1}{c}{}                                & {Range} & \textbf{\color[HTML]{036400}{83.7\%}} & \textbf{\color[HTML]{036400}{85.1\%}} & \textbf{\color[HTML]{036400}{82.9\%}} & \textbf{\color[HTML]{036400}{86.1\%}} & \textbf{\color[HTML]{036400}{86.7\%}} & {} & \textbf{\color[HTML]{036400}{84.9\%}} \\ \hline
\multicolumn{1}{c}{\multirow{3}{*}{{$Z_3$}}} & {Max}   & 299949          & 29488           & 28154           & 31445           & 30055           &           & 29818.2         \\ 
\multicolumn{1}{c}{}                                & {Min}   & 4096            & 4288            & 4298            & 4652            & 4102            &           & 4287.2          \\ 
\multicolumn{1}{c}{}                                & {Range} & \textbf{\color[HTML]{036400}{86.3\%}} & \textbf{\color[HTML]{036400}{85.5\%}} & \textbf{\color[HTML]{036400}{84.7\%}} & \textbf{\color[HTML]{036400}{85.2\%}} & \textbf{\color[HTML]{036400}{86.4\%}} & {} & \textbf{\color[HTML]{036400}{85.6\%}} \\ \hline
\multicolumn{1}{c}{\multirow{3}{*}{{$Z_4$}}} & {Max}   & 30040           & 30478           & 30063           & 31103           & 29206           &           & 30178.0         \\ 
\multicolumn{1}{c}{}                                & {Min}   & 5075            & 3749            & 3673            & 4334            & 4563            &           & 4278.8          \\ 
\multicolumn{1}{c}{}                                & {Range} & \textbf{\color[HTML]{036400}{83.1\%}} & \textbf{\color[HTML]{036400}{87.7\%}} & \textbf{\color[HTML]{036400}{87.8\%}} & \textbf{\color[HTML]{036400}{86.1\%}} & \textbf{\color[HTML]{036400}{84.4\%}} & {} & \textbf{\color[HTML]{036400}{85.8\%}} \\ \hline
\end{tabular}
}
%\subcaption{Set X}
\label{s2X}
\end{subtable}
\caption{Results for the objective ranges analysis.}
\label{step2}
\end{table}

==> figures/step3.tex <==
\begin{table}[!ht]
\centering
\begin{subtable}{0.49\linewidth}
\resizebox{\linewidth}{!}{%
\begin{tabular}{r|c|c|c|c|r}
\multicolumn{1}{c}{} & \multicolumn{2}{c|}{$Z_2^\text{\tiny \leftthumbsup}$} & \multicolumn{2}{c}{$Z_2^\text{\tiny \leftthumbsdown}$} &  \bigstrut[b]\\ \hhline{|~|-|-|-|-|}
\cline{2-5}\multicolumn{1}{c|}{\multirow{2}[4]{*}{$Z_4^\text{\tiny \leftthumbsup}$}} & 0.0\% & {\cellcolor[HTML]{EFEFEF}{4.4\%}} & {\cellcolor[HTML]{C0C0C0}{8.7\%}} & {\cellcolor[HTML]{EFEFEF}{0.5\%}} & \multicolumn{1}{c}{$Z_3^\text{\tiny \leftthumbsup}$} \bigstrut\\ \hhline{|~|-|-|-|-|}
\cline{2-6}\multicolumn{1}{c|}{} & {\cellcolor[HTML]{EFEFEF}{0.1\%}} & {\cellcolor[HTML]{C0C0C0}{6.5\%}} & {\cellcolor[HTML]{9B9B9B}{11.6\%}} & {\cellcolor[HTML]{C0C0C0}{4.6\%}} & \multicolumn{1}{c}{\multirow{2}[4]{*}{$Z_3^\text{\tiny \leftthumbsdown}$}} \bigstrut\\ \hhline{|~|-|-|-|-|}
\cline{1-5}\multicolumn{1}{c|}{\multirow{2}[4]{*}{$Z_4^\text{\tiny \leftthumbsdown}$}} & {\cellcolor[HTML]{C0C0C0}{0.3\%}} & {\cellcolor[HTML]{9B9B9B}{8.5\%}} & {\cellcolor[HTML]{656565}{\color[HTML]{FFFFFF}7.4\%}} & {\cellcolor[HTML]{9B9B9B}{5.3\%}} & \multicolumn{1}{c}{} \bigstrut\\ \hhline{|~|-|-|-|-|}
\cline{2-6}\multicolumn{1}{c|}{} & {\cellcolor[HTML]{EFEFEF}{0.9\%}} & {\cellcolor[HTML]{C0C0C0}{10.5\%}} & {\cellcolor[HTML]{9B9B9B}{@15@\%}} & {\cellcolor[HTML]{C0C0C0}{@16@\%}} & \multicolumn{1}{c}{$Z_3^\text{\tiny \leftthumbsup}$} \bigstrut\\ \hhline{|~|-|-|-|-|}
\cline{2-5}\multicolumn{1}{r}{} & $Z_1^\text{\tiny \leftthumbsdown}$     & \multicolumn{2}{c|}{$Z_1^\text{\tiny \leftthumbsdown}$} & \multicolumn{1}{c}{$Z_1^\text{\tiny \leftthumbsup}$} &  \bigstrut[t]\\
\end{tabular}%
}
\subcaption{Set A}
\label{s3A}
\end{subtable}
\hfill
\begin{subtable}{0.49\linewidth}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cc|c|c|cc}
 & \multicolumn{2}{c|}{\textbf{$Z_2^\text{\tiny \leftthumbsup}$}} &
 \multicolumn{2}{c}{\textbf{$Z_2^\text{\tiny \leftthumbsdown}$}} &  \\ \hhline{~----}
\multicolumn{1}{c|}{} 
& 45.0\% 
& \cellcolor[HTML]{EFEFEF}10.0\% 
& \cellcolor[HTML]{C0C0C0}11.7\% 
& \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}00.0\%} & \textbf{$Z_3^\text{\tiny \leftthumbsup}$} \\ \hhline{~-----}
\multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{$Z_4^\text{\tiny \leftthumbsup}$}}} 
& \cellcolor[HTML]{EFEFEF}00.0\% 
& \cellcolor[HTML]{C0C0C0}00.0\% 
& \cellcolor[HTML]{9B9B9B}00.0\%
& \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}00.0\%} &  \\ \hhline{-----}
\multicolumn{1}{c|}{} 
& \cellcolor[HTML]{C0C0C0}13.3\% 
& \cellcolor[HTML]{9B9B9B}00.0\% 
& \cellcolor[HTML]{656565}{\color{white}00.0\%}
& \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}15.0\%} & \multirow{-2}{*}{\textbf{$Z_3^\text{\tiny \leftthumbsdown}$}} \\ \hhline{~-----}
\multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{$Z_4^\text{\tiny \leftthumbsdown}$}}} 
& \cellcolor[HTML]{EFEFEF}00.0\% 
& \cellcolor[HTML]{C0C0C0}00.0\% 
& \cellcolor[HTML]{9B9B9B}05.0\% 
& \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}00.0\%} & \textbf{$Z_3^\text{\tiny \leftthumbsup}$} \\ \hhline{~----}
 & \textbf{$Z_1^\text{\tiny \leftthumbsup}$} & \multicolumn{2}{c|}{\textbf{$Z_1^\text{\tiny \leftthumbsdown}$}} & \textbf{$Z_1^\text{\tiny \leftthumbsup}$} & 
\end{tabular}
}
\subcaption{Set B}
\label{s3B}
\end{subtable}
\\
\begin{subtable}{0.49\linewidth}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cc|c|c|cc}
 & \multicolumn{2}{c|}{\textbf{$Z_2^\text{\tiny \leftthumbsup}$}} &
 \multicolumn{2}{c}{\textbf{$Z_2^\text{\tiny \leftthumbsdown}$}} &  \\ \hhline{~----}
\multicolumn{1}{c|}{} 
& 00.0\% 
& \cellcolor[HTML]{EFEFEF}00.2\% 
& \cellcolor[HTML]{C0C0C0}00.3\% 
& \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}00.6\%} & \textbf{$Z_3^\text{\tiny \leftthumbsup}$} \\ \hhline{~-----}
\multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{$Z_4^\text{\tiny \leftthumbsup}$}}} 
& \cellcolor[HTML]{EFEFEF}00.0\% 
& \cellcolor[HTML]{C0C0C0}49.9\% 
& \cellcolor[HTML]{9B9B9B}01.9\%
& \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}00.3\%} &  \\ \hhline{-----}
\multicolumn{1}{c|}{} 
& \cellcolor[HTML]{C0C0C0}00.0\% 
& \cellcolor[HTML]{9B9B9B}00.9\% 
& \cellcolor[HTML]{656565}{\color{white}00.8\%} 
& \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}00.4\%} & \multirow{-2}{*}{\textbf{$Z_3^\text{\tiny \leftthumbsdown}$}} \\ \hhline{~-----}
\multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{$Z_4^\text{\tiny \leftthumbsdown}$}}} 
& \cellcolor[HTML]{EFEFEF}00.0\% 
& \cellcolor[HTML]{C0C0C0}00.2\% 
& \cellcolor[HTML]{9B9B9B}00.8\% 
& \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}43.5\%} & \textbf{$Z_3^\text{\tiny \leftthumbsup}$} \\ \hhline{~----}
 & \textbf{$Z_1^\text{\tiny \leftthumbsup}$} & \multicolumn{2}{c|}{\textbf{$Z_1^\text{\tiny \leftthumbsdown}$}} & \textbf{$Z_1^\text{\tiny \leftthumbsup}$} & 
\end{tabular}
}
\subcaption{Set C}
\label{s3C}
\end{subtable}
\hfill
\begin{subtable}{0.49\linewidth}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cc|c|c|cc}
 & \multicolumn{2}{c|}{\textbf{$Z_2^\text{\tiny \leftthumbsup}$}} &
 \multicolumn{2}{c}{\textbf{$Z_2^\text{\tiny \leftthumbsdown}$}} &  \\ \hhline{~----}
\multicolumn{1}{c|}{} 
& 00.0\% 
& \cellcolor[HTML]{EFEFEF}00.0\% 
& \cellcolor[HTML]{C0C0C0}00.0\% 
& \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}00.0\%} & \textbf{$Z_3^\text{\tiny \leftthumbsup}$} \\ \hhline{~-----}
\multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{$Z_4^\text{\tiny \leftthumbsup}$}}} 
& \cellcolor[HTML]{EFEFEF}00.0\% 
& \cellcolor[HTML]{C0C0C0}55.6\% 
& \cellcolor[HTML]{9B9B9B}04.7\%
& \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}00.0\%} &  \\ \hhline{-----}
\multicolumn{1}{c|}{} 
& \cellcolor[HTML]{C0C0C0}00.0\% 
& \cellcolor[HTML]{9B9B9B}04.4\% 
& \cellcolor[HTML]{656565}{\color{white}09.9\%}
& \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}01.8\%} & \multirow{-2}{*}{\textbf{$Z_3^\text{\tiny \leftthumbsdown}$}} \\ \hhline{~-----} 
\multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{$Z_4^\text{\tiny \leftthumbsdown}$}}} 
& \cellcolor[HTML]{EFEFEF}00.0\% 
& \cellcolor[HTML]{C0C0C0}00.0\% 
& \cellcolor[HTML]{9B9B9B}01.0\% 
& \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}22.6\%} & \textbf{$Z_3^\text{\tiny \leftthumbsup}$} \\ \hhline{~----}
 & \textbf{$Z_1^\text{\tiny \leftthumbsup}$} & \multicolumn{2}{c|}{\textbf{$Z_1^\text{\tiny \leftthumbsdown}$}} & \textbf{$Z_1^\text{\tiny \leftthumbsup}$} & 
\end{tabular}
}
\subcaption{Set D}
\label{s3D}
\end{subtable}
\\
\begin{subtable}{0.49\linewidth}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cc|c|c|cc}
 & \multicolumn{2}{c|}{\textbf{$Z_2^\text{\tiny \leftthumbsup}$}} &
 \multicolumn{2}{c}{\textbf{$Z_2^\text{\tiny \leftthumbsdown}$}} &  \\ \hhline{~----}
\multicolumn{1}{c|}{} 
& 00.0\% 
& \cellcolor[HTML]{EFEFEF}00.0\% 
& \cellcolor[HTML]{C0C0C0}05.9\% 
& \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}00.0\%} & \textbf{$Z_3^\text{\tiny \leftthumbsup}$} \\ \hhline{~-----}
\multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{$Z_4^\text{\tiny \leftthumbsup}$}}} 
& \cellcolor[HTML]{EFEFEF}00.0\% 
& \cellcolor[HTML]{C0C0C0}06.2\% 
& \cellcolor[HTML]{9B9B9B}10.0\%
& \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}05.9\%} &  \\ \hhline{-----}
\multicolumn{1}{c|}{} 
& \cellcolor[HTML]{C0C0C0}07.9\% 
& \cellcolor[HTML]{9B9B9B}15.4\% 
& \cellcolor[HTML]{656565}{\color{white}04.7\%}
& \multicolumn{1}{c|}{\cellcolor[HTML]{9B9B9B}15.0\%} & \multirow{-2}{*}{\textbf{$Z_3^\text{\tiny \leftthumbsdown}$}} \\ \hhline{~-----}
\multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{$Z_4^\text{\tiny \leftthumbsdown}$}}} 
& \cellcolor[HTML]{EFEFEF}00.0\% 
& \cellcolor[HTML]{C0C0C0}07.1\% 
& \cellcolor[HTML]{9B9B9B}15.4\% 
& \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}06.4\%} & \textbf{$Z_3^\text{\tiny \leftthumbsup}$} \\ \hhline{~----}
 & \textbf{$Z_1^\text{\tiny \leftthumbsup}$} & \multicolumn{2}{c|}{\textbf{$Z_1^\text{\tiny \leftthumbsdown}$}} & \textbf{$Z_1^\text{\tiny \leftthumbsup}$} & 
\end{tabular}
}
\subcaption{Set X}
\label{s3X}
\end{subtable}
\caption{Results for the trade-off regions analysis.}
\label{step3}
\end{table}
